TLCFuse: Temporal Multi-Modality Fusion Towards Occlusion-Aware Semantic Segmentation-Aided Motion Planning

In autonomous driving, addressing occlusion scenarios is crucial yet challenging. Robust surrounding perception is essential for handling occlusions and aiding motion planning. State-of-the-art models fuse Lidar and Camera data to produce impressive perception results, but detecting occluded objects remains challenging. In this paper, we emphasize the crucial role of temporal cues by integrating them alongside these modalities to address this challenge. We propose a novel approach for bird's eye view semantic grid segmentation, that leverages sequential sensor data to achieve robustness against occlusions. Our model extracts information from the sensor readings using attention operations and aggregates this information into a lower-dimensional latent representation, enabling thus the processing of multi-step inputs at each prediction step. Moreover, we show how it can also be directly applied to forecast the development of traffic scenes and be seamlessly integrated into a motion planner for trajectory planning. On the semantic segmentation tasks, we evaluate our model on the nuScenes dataset and show that it outperforms other baselines, with particularly large differences when evaluating on occluded and partially-occluded vehicles. Additionally, on motion planning task we are among the early teams to train and evaluate on nuPlan, a cutting-edge large-scale dataset for motion planning.

==> sections/ablation.tex <==
%!TEX root = ../main.tex


% \section{Ablation studies} \label{sec:ablation}
\subsection{Ablation Study}
Table \ref{tab:ablation} shows the ablation study on the various input modalities of our proposed network.

% \textbf{Ablation studies for temporal fusion.} We first conduct an ablation study towards our temporal fusion technique. To simplify the procedure, we use only camera frames as input, predict single step BEV grid with visibility $\geq$ 0\%. We use a temporal sequence length(Seq) of 3 or 4 frames as our input, which represents 1 or 1.5 seconds in the past respectively. And we set the number of self-attention layers used(SA) following each cross-attention layer to 2 or 4. The IOU scores are displayed in Table \ref{tab:ablation}. 

% \begin{table}[th]
% \fontsize{9}{11}\selectfont
% \centering
% \begin{tabular}{ccccccc}
% \hline
% Seq & SA & Arch. & egomotion  & VH & DA \\ \hline
% 3            & 4              & Series        & \xmark    &        34.82          &  \textbf{75.86}  \\
% 3            & 2              & Series        & \xmark    &        35.40          &  74.06  \\
% 3            & 2              & Series        & \cmark    &        \textbf{35.67} &  75.71  \\
% 3            & 4              & Parallel      & \xmark    &        31.31          &  73.82  \\
% 3            & 2              & Parallel      & \xmark    &        31.39          &  73.38  \\
% 3            & 2              & Series-Residual        & \cmark    &        35.31 &  74.96  \\
% 4            & 4              & Series        & \xmark    &        33.38          &  73.54  \\
% 4            & 2              & Series        & \xmark    &        34.22          &  72.44  \\ \hline
% \end{tabular}
% \caption{\textbf{Ablation studies for temporal fusion.} IOU scores from different temporal architectures tested with only camera frames as input. Seq(sequence length) indicates the number of frames (n) used $(t ... t_{n-1})$. SA indicates the number of Self-attention layers used. In some cases the egomotion information is concatenated to the input features. VH: Vehicles class. DA: Drivable Area class.}
% \label{tab:ablation}
% %\vspace{-0.3em}
% \end{table}

% From the resultant scores within Table \ref{tab:ablation}, we learn that using 3 input time steps gives better results than with 4, and 2 SA layers better than 4. This could be due to the fact that with longer input temporal horizon and bigger model, the model aggregates more recent data and gradually forgets the oldest input features(e.g. $t_{-2}$). To tackle such memory disappearing issue, a model with residual connections is evaluated where the temporal features are skipped connections and added to the following ones, similar to the residual architecture \cite{he2016deep}. This model presents positive results, although it is not the best scores obtained.

% Additionally, we also evaluate the effect of warping the input features from past timestamps to the current reference time, by concatenating the egomotion information(the translation and rotation from past to present) to the input features. From the scores, the models that are trained using this composed input showing improvement over all the others.

% As a conclusion, the best IOU score of 35.67 for visibility $\geq$ 0\% is achieved by the model with temporal architecture in series, temporal sequence length of 3 frames, 2 layers of self-attention with egomotion embedding attached to the input features.%This model as seen in Table \ref{tab:ablation} outperforms the others with the IOU score 35.67 for visibility $\geq$ 0\%.% and 37.80 for visibility $>$ 40\%.

% \begin{table}[b!]
% \fontsize{8.7}{10.7}\selectfont
% \centering
% \begin{tabular}{lccc}
% \hline
% Method                    & vis $\geq$ 0\%       & vis $>$  40\%       & 0\% $<$ vis $<$ 40\% \\ \hline
% LaRa (C)             &     35.81            &     37.92             &      25.81                       \\
% LaRa (L)              &     31.09            &     32.63             &      24.05                       \\
% LaRa (C+L)     &     42.56            &     44.94             &      31.90                       \\
% TLCFuse (C)         &     35.67            &     37.80             &      25.77                       \\
% TLCFuse (L)          &     32.01            &     33.38             &      25.76                       \\
% \textbf{TLCFuse (C+L)} &     \textbf{43.65}   &     \textbf{46.40}    &      \textbf{32.69}              \\ \hline
% \end{tabular}
% \caption{\textbf{Ablation studies with different visibility levels.} IOU results comparing TLCFuse with LaRa model, for vehicles visibility levels: visibility greater than 0\%, visibility greater than 40\% and visibility between 0\% and 40\%.}
% \label{tab:vis123}
% \vspace{-1.2em}
% \end{table}


\begin{table}[h]
\begin{adjustbox}{width=\columnwidth,center}
\centering
\begin{tabular}{c|ccc|ccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{ID}}  & \multicolumn{3}{c|}{Modality} & \multicolumn{3}{c}{IoU}\\
\multicolumn{1}{c|}{}                     & Camera   & LiDAR   & Temporal &  vis $\geq$ 0\%  & vis $>$  40\%  & 0\% $<$ vis $<$ 40\% \\  \hline
1                                         & \checkmark   &     &          &  35.61           & 37.92          &                       \\
2                                         &        &\checkmark &          & 31.09            &32.63           &                       \\
3                                         &\checkmark  & \checkmark &     & 42.56            & 44.94          &                   \\
4                                         & \checkmark &       &\checkmark& 35.67            &37.80            &                       \\ 
5                                         &  & \checkmark      &\checkmark& 32.01           &33.38           &                       \\                    6                                         & \checkmark & \checkmark  &\checkmark  & \textbf{43.65}      & \textbf{46.40 }      &            \\ \hline      
\end{tabular}
\end{adjustbox}
\caption{\textbf{Ablation on different modalities.} We show here the BEV segmentation results using different input modalities.}
\label{tab:ablation}
\vspace{-0.3em}
\end{table}


\textbf{Ablation studies with different visibility levels.} 
Table \ref{tab:ablation} shows the IOU performances for the ablation studies over different input data modalities across different levels of visibility of the vehicles. We take the state-of-art camera-only model for BEV semantic grid generation, LaRa \cite{bartoccioni2022lara} as our comparison. We modify the original code base provided by LaRa to be able to train and test with lidar-only or lidar-camera fused input modality setups. During training, all the vehicles with or without occlusion from the training set are used. While during validating, we report IOU scores for 3 different visibility levels. For the visibility greater than 0\% (second column in the table), all the vehicles within the scenes of the validation set are used. For visibility greater than 40\% (third column in the table), only the visible vehicles (not significantly occluded) in the ground truth included. Lastly, the visibility between 0\% and 40\% (fourth column in the table), only partially or completely occluded vehicles in the ground truth are used. From the table, the scores suggest that fusing Lidar and camera data outperforms single modality models. Adding temporal information further boosts the performance, making our proposed TLCFuse the best model among all. Furthermore, the strength of TLCFuse is specifically more obvious in the BEV semantic grid prediction of the occluded vehicles.

% We can see that the proposed method using Camera, Lidar and temporal context information outperforms all others. Next, for visibility greater than 40\% the vehicles in the ground truth are no longer (significantly) occluded; here TLCFuse also outperforms all other models. By analyzing the scores it is possible to observe patterns that suggest that the fusion of both modalities lead to superior performance, and that the camera-only input presents better results than the Lidar-only input for both architectures. Finally, the visibility between 0\% and 40\% tells us how well the models perform in the segmentation of occluded vehicles. %, as the ground truth brings totally/significantly occluded cars.
% The scores show the advantage of leveraging camera and Lidar input modalities as well as the temporal context.% as TLCFuse(C+L) scores 32.69.

%explain table II ...

%explain results of ablation
